Data-Driven Spectral Submanifold Reduction for Nonlinear Optimal Control of High-Dimensional Robots

Modeling and control of high-dimensional, nonlinear robotic systems remains a challenging task. While various model- and learning-based approaches have been proposed to address these challenges, they broadly lack generalizability to different control tasks and rarely preserve the structure of the dynamics. In this work, we propose a new, data-driven approach for extracting low-dimensional models from data using Spectral Submanifold Reduction (SSMR). In contrast to other data-driven methods which fit dynamical models to training trajectories, we identify the dynamics on generic, low-dimensional attractors embedded in the full phase space of the robotic system. This allows us to obtain computationally-tractable models for control which preserve the system's dominant dynamics and better track trajectories radically different from the training data. We demonstrate the superior performance and generalizability of SSMR in dynamic trajectory tracking tasks vis-a-vis the state of the art, including Koopman operator-based approaches.

==> Data-Driven Spectral Submanifold Reduction for Nonlinear Optimal Control of High-Dimensional Robots/commands.tex <==
\usepackage{mathtools}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

% notes
\newcommand{\john}[1]{{\color{red}{JA: #1}}}
\newcommand{\spencer}[1]{{\color{red}{SR: #1}}}
\newcommand{\mattia}[1]{{\color{red}{MC: #1}}}

% theorem blocks
\newtheorem{defn}{Definition}
\newtheorem{rem}[defn]{Remark}
\newtheorem{lem}[defn]{Lemma}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{assum}[defn]{Assumption}
\newtheorem{ex}[defn]{Example}
\newtheorem{thm}[defn]{Theorem}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{prob}{Problem}

% important sets
\providecommand{\R}{\ensuremath \mathbb{R}}
\providecommand{\Z}{\ensuremath \mathbb{Z}}
\providecommand{\N}{\ensuremath \mathbb{N}}
\newcommand{\SE}{\regtext{SE}}
\newcommand{\SO}{\regtext{SO}}

% useful text modifications
\newcommand{\regtext}[1]{\mathrm{\textnormal{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ts}[1]{\textsuperscript{#1}}
\newcommand{\ie}{\textit{i.e., }}
\newcommand{\eg}{\textit{e.g., }}


% common operations
\newcommand{\comp}{^{\regtext{C}}}
\newcommand{\card}[1]{\left\vert#1\right\vert}
\newcommand{\interior}[1]{\regtext{int}\!\left(#1\right)}
\newcommand{\proj}{\regtext{proj}}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\pow}[1]{\regtext{pow}\!\left(#1\right)}
\newcommand{\diag}[1]{\regtext{diag}\!\left(#1\right)}
\newcommand{\eig}[1]{\regtext{eig}\!\left(#1\right)}
\newcommand{\union}{\bigcup}
\newcommand{\intersection}{\bigcap}
\newcommand{\trans}{^\top}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\sign}{\regtext{sign}}
\newcommand{\expm}{\regtext{exp}}
\newcommand{\logm}{\regtext{log}}
\newcommand{\skw}{_{\times}}
\newcommand{\bigO}{\pazocal{O}}
\newcommand{\bdry}[1]{{\partial #1}}
\renewcommand{\ker}[1]{\regtext{ker}\!\left(#1\right)}
\newcommand{\convhull}[1]{\regtext{CH}\!\left(#1\right)}
\newcommand{\dist}[1]{d_2\!\left(#1\right)}
\newcommand{\len}[1]{\left\Vert#1\right\Vert_2}
\newcommand{\trace}{\regtext{trace}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\derive}{\mathrm{D}}



% math types
% \newcommand{\vc}[1]{\mathbf{#1}}
% \newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\vect}[1]{#1}
\newcommand{\mat}[1]{#1}
\newcommand{\set}[1]{\mathbb{#1}}



% generic math objects
\newcommand{\normaldist}{\mathscr{N}}
\newcommand{\vep}{\varepsilon}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}} %Spectral subspace
\newcommand{\real}{\mathrm{Re}}
\newcommand{\imag}{\mathrm{Im}}
\newcommand{\Spec}{\mathrm{Spect}}
\DeclareMathOperator*{\minimize}{\mathrm{minimize}}
\DeclareMathOperator*{\subjectto}{\mathrm{subject~to}}
\DeclareMathOperator*{\argmin}{arg\,min}


% labels
\newcommand{\goal}{{\regtext{goal}}}
\newcommand{\ego}{{\regtext{e}}}


% special arrays
\newcommand{\emptyarr}{[\ ]}
\newcommand{\zeros}{{0}}
\newcommand{\ones}{{1}}
\newcommand{\eye}{{I}}


% indexing
% \newcommand{\idx}[1]{{\langle#1\rangle}} % index an element of a set
\newcommand{\idx}[1]{^{(#1)}} % index an element of a set
% \newcommand{\arridx}[1]{{[#1]}} % index elements of an array/vector

% paper-relevant objects

\providecommand{\Torus}{\ensuremath \mathbb{T}}
\newcommand{\fstate}{\mathbf{x}^{f}}
\newcommand{\rstate}{\mathbf{x}}
\newcommand{\perf}{\mathbf{z}}
\newcommand{\obs}{\mathbf{y}}
\newcommand{\perfref}{\bar{\perf}}
\newcommand{\outrefphase}{z^\star}
\newcommand{\phase}{\vect{\varphi}}
\newcommand{\freq}{\vect{\omega}} 
\newcommand{\ctrltaylor}{\vect{D}}
\newcommand{\ssm}{\vect{W}}
\newcommand{\rdyn}{\vect{R}}
\newcommand{\nnm}{\gamma_{\epsilon}}
\newcommand{\autSSM}{\pazocal{W}(E)}
\newcommand{\nonautSSM}{\mathcal{W}(E,\nnm)}

\newcommand{\mass}{\mathbf{M}}
\newcommand{\damp}{\mathbf{C}}
\newcommand{\stiff}{\mathbf{K}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\ctrl}{\mathbf{u}}
\newcommand{\Cntrl}{\pazocal{U}}
\newcommand{\Observable}{\pazocal{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Qf}{\mathbf{Q}_{\mathrm{f}}}
\newcommand{\Rcost}{\mathbf{R}}
\newcommand{\spectralsubspace}{E}
\newcommand{\ytox}{\mathbf{v}}
\newcommand{\xtoy}{\mathbf{w}}
\newcommand{\truncidx}{\bar{k}}
\newcommand{\Ydata}{\mathbfcal{Y}}
\newcommand{\X}{\mathbfcal{X}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\Br}{\mathbf{B}_r}





% % sizes of things
\newcommand{\nfstate}{{n_{f}}}
\newcommand{\nrstate}{n}
\newcommand{\nctrl}{m}
\newcommand{\nperf}{o}
\newcommand{\nout}{p}
\newcommand{\nfreq}{1}
\newcommand{\phasedom}{S^1}
\newcommand{\freqdom}{\R_+}
% for quasi-periodic setting change to:
% \newcommand{\nfreq}{K}
% \newcommand{\phasedom}{\Torus^\nfreq}
% \newcommand{\freqdom}{\R_+^\nfreq}
\newcommand{\nctrltaylor}{\Upsilon}
\newcommand{\nctrlfourier}{\Gamma}
\newcommand{\nodes}{\pazocal{N}}


% \newcommand{\state}{x}
% \newcommand{\mode}{z}
% \newcommand{\ctrl}{u}
% \newcommand{\noise}{w}
% \newcommand{\horizon}{t_{\regtext{f}}}
% \newcommand{\horizondisc}{k_{\regtext{f}}}
% \newcommand{\at}[1]{\!\left(#1\right)}
% \newcommand{\dt}{\Delta_t}

% \newcommand{\zonotope}{\set{Z}}
% \newcommand{\reachset}{\set{X}}
% \newcommand{\noisespace}{\set{W}}

% \newcommand{\statehistory}{X}
% \newcommand{\ctrlhistory}{U}

% % sizes of things
% \newcommand{\nstate}{{n_\state}}
% \newcommand{\nctrl}{{n_\ctrl}}
% \newcommand{\nnoise}{{n_\noise}}
% \newcommand{\nagents}{{n_{\regtext{a}}}}
% \newcommand{\nmodes}{{n_{\regtext{m}}}}
% \newcommand{\nego}{{n_{\ego}}}
% \newcommand{\ngen}{{n_{\regtext{g}}}}
% \newcommand{\ncon}{{n_{\regtext{c}}}}

% % zonotope stuff
% \newcommand{\zonofn}[1]{{\mathscr{Z}\!\left(#1\right)}}

% % MATS
% \newcommand{\MATS}{\phi}
% \newcommand{\param}{\theta}

==> Data-Driven Spectral Submanifold Reduction for Nonlinear Optimal Control of High-Dimensional Robots/figures/Dynamics-based Machine Learning for Nonlinear Model Predictive Control of Soft Robots/commands.tex <==
\usepackage{mathtools}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

% notes
\newcommand{\john}[1]{{\color{red}{JA: #1}}}
\newcommand{\spencer}[1]{{\color{red}{SR: #1}}}
\newcommand{\mattia}[1]{{\color{red}{MC: #1}}}

% theorem blocks
\newtheorem{defn}{Definition}
\newtheorem{rem}[defn]{Remark}
\newtheorem{lem}[defn]{Lemma}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{assum}[defn]{Assumption}
\newtheorem{ex}[defn]{Example}
\newtheorem{thm}[defn]{Theorem}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{prob}{Problem}

% important sets
\providecommand{\R}{\ensuremath \mathbb{R}}
\providecommand{\Z}{\ensuremath \mathbb{Z}}
\providecommand{\N}{\ensuremath \mathbb{N}}
\newcommand{\SE}{\regtext{SE}}
\newcommand{\SO}{\regtext{SO}}

% useful text modifications
\newcommand{\regtext}[1]{\mathrm{\textnormal{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ts}[1]{\textsuperscript{#1}}
\newcommand{\ie}{\textit{i.e., }}
\newcommand{\eg}{\textit{e.g., }}


% common operations
\newcommand{\comp}{^{\regtext{C}}}
\newcommand{\card}[1]{\left\vert#1\right\vert}
\newcommand{\interior}[1]{\regtext{int}\!\left(#1\right)}
\newcommand{\proj}{\regtext{proj}}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\pow}[1]{\regtext{pow}\!\left(#1\right)}
\newcommand{\diag}[1]{\regtext{diag}\!\left(#1\right)}
\newcommand{\eig}[1]{\regtext{eig}\!\left(#1\right)}
\newcommand{\union}{\bigcup}
\newcommand{\intersection}{\bigcap}
\newcommand{\trans}{^\top}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\sign}{\regtext{sign}}
\newcommand{\expm}{\regtext{exp}}
\newcommand{\logm}{\regtext{log}}
\newcommand{\skw}{_{\times}}
\newcommand{\bigO}{\pazocal{O}}
\newcommand{\bdry}[1]{{\partial #1}}
\renewcommand{\ker}[1]{\regtext{ker}\!\left(#1\right)}
\newcommand{\convhull}[1]{\regtext{CH}\!\left(#1\right)}
\newcommand{\dist}[1]{d_2\!\left(#1\right)}
\newcommand{\len}[1]{\left\Vert#1\right\Vert_2}
\newcommand{\trace}{\regtext{trace}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\derive}{\mathrm{D}}



% math types
% \newcommand{\vc}[1]{\mathbf{#1}}
% \newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\vect}[1]{#1}
\newcommand{\mat}[1]{#1}
\newcommand{\set}[1]{\mathbb{#1}}



% generic math objects
\newcommand{\normaldist}{\mathscr{N}}
\newcommand{\vep}{\varepsilon}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}} %Spectral subspace
\newcommand{\real}{\mathrm{Re}}
\newcommand{\imag}{\mathrm{Im}}
\newcommand{\Spec}{\mathrm{Spect}}
\DeclareMathOperator*{\minimize}{\mathrm{minimize}}
\DeclareMathOperator*{\subjectto}{\mathrm{subject~to}}
\DeclareMathOperator*{\argmin}{arg\,min}


% labels
\newcommand{\goal}{{\regtext{goal}}}
\newcommand{\ego}{{\regtext{e}}}


% special arrays
\newcommand{\emptyarr}{[\ ]}
\newcommand{\zeros}{{0}}
\newcommand{\ones}{{1}}
\newcommand{\eye}{{I}}


% indexing
% \newcommand{\idx}[1]{{\langle#1\rangle}} % index an element of a set
\newcommand{\idx}[1]{^{(#1)}} % index an element of a set
% \newcommand{\arridx}[1]{{[#1]}} % index elements of an array/vector

% paper-relevant objects

\providecommand{\Torus}{\ensuremath \mathbb{T}}
\newcommand{\fstate}{\mathbf{x}^{f}}
\newcommand{\rstate}{\mathbf{x}}
\newcommand{\perf}{\mathbf{z}}
\newcommand{\obs}{\mathbf{y}}
\newcommand{\perfref}{\bar{\perf}}
\newcommand{\outrefphase}{z^\star}
\newcommand{\phase}{\vect{\varphi}}
\newcommand{\freq}{\vect{\omega}} 
\newcommand{\ctrltaylor}{\vect{D}}
\newcommand{\ssm}{\vect{W}}
\newcommand{\rdyn}{\vect{R}}
\newcommand{\nnm}{\gamma_{\epsilon}}
\newcommand{\autSSM}{\pazocal{W}(E)}
\newcommand{\nonautSSM}{\mathcal{W}(E,\nnm)}

\newcommand{\mass}{\mathbf{M}}
\newcommand{\damp}{\mathbf{C}}
\newcommand{\stiff}{\mathbf{K}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\ctrl}{\mathbf{u}}
\newcommand{\Cntrl}{\pazocal{U}}
\newcommand{\Observable}{\pazocal{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Qf}{\mathbf{Q}_{\mathrm{f}}}
\newcommand{\Rcost}{\mathbf{R}}
\newcommand{\spectralsubspace}{E}
\newcommand{\ytox}{\mathbf{v}}
\newcommand{\xtoy}{\mathbf{w}}
\newcommand{\truncidx}{\bar{k}}
\newcommand{\Ydata}{\mathbfcal{Y}}
\newcommand{\X}{\mathbfcal{X}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\Br}{\mathbf{B}_r}





% % sizes of things
\newcommand{\nfstate}{{n_{f}}}
\newcommand{\nrstate}{n}
\newcommand{\nctrl}{m}
\newcommand{\nperf}{o}
\newcommand{\nout}{p}
\newcommand{\nfreq}{1}
\newcommand{\phasedom}{S^1}
\newcommand{\freqdom}{\R_+}
% for quasi-periodic setting change to:
% \newcommand{\nfreq}{K}
% \newcommand{\phasedom}{\Torus^\nfreq}
% \newcommand{\freqdom}{\R_+^\nfreq}
\newcommand{\nctrltaylor}{\Upsilon}
\newcommand{\nctrlfourier}{\Gamma}
\newcommand{\nodes}{\pazocal{N}}


% \newcommand{\state}{x}
% \newcommand{\mode}{z}
% \newcommand{\ctrl}{u}
% \newcommand{\noise}{w}
% \newcommand{\horizon}{t_{\regtext{f}}}
% \newcommand{\horizondisc}{k_{\regtext{f}}}
% \newcommand{\at}[1]{\!\left(#1\right)}
% \newcommand{\dt}{\Delta_t}

% \newcommand{\zonotope}{\set{Z}}
% \newcommand{\reachset}{\set{X}}
% \newcommand{\noisespace}{\set{W}}

% \newcommand{\statehistory}{X}
% \newcommand{\ctrlhistory}{U}

% % sizes of things
% \newcommand{\nstate}{{n_\state}}
% \newcommand{\nctrl}{{n_\ctrl}}
% \newcommand{\nnoise}{{n_\noise}}
% \newcommand{\nagents}{{n_{\regtext{a}}}}
% \newcommand{\nmodes}{{n_{\regtext{m}}}}
% \newcommand{\nego}{{n_{\ego}}}
% \newcommand{\ngen}{{n_{\regtext{g}}}}
% \newcommand{\ncon}{{n_{\regtext{c}}}}

% % zonotope stuff
% \newcommand{\zonofn}[1]{{\mathscr{Z}\!\left(#1\right)}}

% % MATS
% \newcommand{\MATS}{\phi}
% \newcommand{\param}{\theta}

==> figures/Dynamics-based Machine Learning for Nonlinear Model Predictive Control of Soft Robots/commands.tex <==
\usepackage{mathtools}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

% notes
\newcommand{\john}[1]{{\color{red}{JA: #1}}}
\newcommand{\spencer}[1]{{\color{red}{SR: #1}}}
\newcommand{\mattia}[1]{{\color{red}{MC: #1}}}

% theorem blocks
\newtheorem{defn}{Definition}
\newtheorem{rem}[defn]{Remark}
\newtheorem{lem}[defn]{Lemma}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{assum}[defn]{Assumption}
\newtheorem{ex}[defn]{Example}
\newtheorem{thm}[defn]{Theorem}
\newtheorem{cor}[defn]{Corollary}
\newtheorem{prob}{Problem}

% important sets
\providecommand{\R}{\ensuremath \mathbb{R}}
\providecommand{\Z}{\ensuremath \mathbb{Z}}
\providecommand{\N}{\ensuremath \mathbb{N}}
\newcommand{\SE}{\regtext{SE}}
\newcommand{\SO}{\regtext{SO}}

% useful text modifications
\newcommand{\regtext}[1]{\mathrm{\textnormal{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ts}[1]{\textsuperscript{#1}}
\newcommand{\ie}{\textit{i.e., }}
\newcommand{\eg}{\textit{e.g., }}


% common operations
\newcommand{\comp}{^{\regtext{C}}}
\newcommand{\card}[1]{\left\vert#1\right\vert}
\newcommand{\interior}[1]{\regtext{int}\!\left(#1\right)}
\newcommand{\proj}{\regtext{proj}}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\pow}[1]{\regtext{pow}\!\left(#1\right)}
\newcommand{\diag}[1]{\regtext{diag}\!\left(#1\right)}
\newcommand{\eig}[1]{\regtext{eig}\!\left(#1\right)}
\newcommand{\union}{\bigcup}
\newcommand{\intersection}{\bigcap}
\newcommand{\trans}{^\top}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\sign}{\regtext{sign}}
\newcommand{\expm}{\regtext{exp}}
\newcommand{\logm}{\regtext{log}}
\newcommand{\skw}{_{\times}}
\newcommand{\bigO}{\pazocal{O}}
\newcommand{\bdry}[1]{{\partial #1}}
\renewcommand{\ker}[1]{\regtext{ker}\!\left(#1\right)}
\newcommand{\convhull}[1]{\regtext{CH}\!\left(#1\right)}
\newcommand{\dist}[1]{d_2\!\left(#1\right)}
\newcommand{\len}[1]{\left\Vert#1\right\Vert_2}
\newcommand{\trace}{\regtext{trace}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\derive}{\mathrm{D}}



% math types
% \newcommand{\vc}[1]{\mathbf{#1}}
% \newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\vect}[1]{#1}
\newcommand{\mat}[1]{#1}
\newcommand{\set}[1]{\mathbb{#1}}



% generic math objects
\newcommand{\normaldist}{\mathscr{N}}
\newcommand{\vep}{\varepsilon}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}} %Spectral subspace
\newcommand{\real}{\mathrm{Re}}
\newcommand{\imag}{\mathrm{Im}}
\newcommand{\Spec}{\mathrm{Spect}}
\DeclareMathOperator*{\minimize}{\mathrm{minimize}}
\DeclareMathOperator*{\subjectto}{\mathrm{subject~to}}
\DeclareMathOperator*{\argmin}{arg\,min}


% labels
\newcommand{\goal}{{\regtext{goal}}}
\newcommand{\ego}{{\regtext{e}}}


% special arrays
\newcommand{\emptyarr}{[\ ]}
\newcommand{\zeros}{{0}}
\newcommand{\ones}{{1}}
\newcommand{\eye}{{I}}


% indexing
% \newcommand{\idx}[1]{{\langle#1\rangle}} % index an element of a set
\newcommand{\idx}[1]{^{(#1)}} % index an element of a set
% \newcommand{\arridx}[1]{{[#1]}} % index elements of an array/vector

% paper-relevant objects

\providecommand{\Torus}{\ensuremath \mathbb{T}}
\newcommand{\fstate}{\mathbf{x}^{f}}
\newcommand{\rstate}{\mathbf{x}}
\newcommand{\perf}{\mathbf{z}}
\newcommand{\obs}{\mathbf{y}}
\newcommand{\perfref}{\bar{\perf}}
\newcommand{\outrefphase}{z^\star}
\newcommand{\phase}{\vect{\varphi}}
\newcommand{\freq}{\vect{\omega}} 
\newcommand{\ctrltaylor}{\vect{D}}
\newcommand{\ssm}{\vect{W}}
\newcommand{\rdyn}{\vect{R}}
\newcommand{\nnm}{\gamma_{\epsilon}}
\newcommand{\autSSM}{\pazocal{W}(E)}
\newcommand{\nonautSSM}{\mathcal{W}(E,\nnm)}

\newcommand{\mass}{\mathbf{M}}
\newcommand{\damp}{\mathbf{C}}
\newcommand{\stiff}{\mathbf{K}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\ctrl}{\mathbf{u}}
\newcommand{\Cntrl}{\pazocal{U}}
\newcommand{\Observable}{\pazocal{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Qf}{\mathbf{Q}_{\mathrm{f}}}
\newcommand{\Rcost}{\mathbf{R}}
\newcommand{\spectralsubspace}{E}
\newcommand{\ytox}{\mathbf{v}}
\newcommand{\xtoy}{\mathbf{w}}
\newcommand{\truncidx}{\bar{k}}
\newcommand{\Ydata}{\mathbfcal{Y}}
\newcommand{\X}{\mathbfcal{X}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\Br}{\mathbf{B}_r}





% % sizes of things
\newcommand{\nfstate}{{n_{f}}}
\newcommand{\nrstate}{n}
\newcommand{\nctrl}{m}
\newcommand{\nperf}{o}
\newcommand{\nout}{p}
\newcommand{\nfreq}{1}
\newcommand{\phasedom}{S^1}
\newcommand{\freqdom}{\R_+}
% for quasi-periodic setting change to:
% \newcommand{\nfreq}{K}
% \newcommand{\phasedom}{\Torus^\nfreq}
% \newcommand{\freqdom}{\R_+^\nfreq}
\newcommand{\nctrltaylor}{\Upsilon}
\newcommand{\nctrlfourier}{\Gamma}
\newcommand{\nodes}{\pazocal{N}}


% \newcommand{\state}{x}
% \newcommand{\mode}{z}
% \newcommand{\ctrl}{u}
% \newcommand{\noise}{w}
% \newcommand{\horizon}{t_{\regtext{f}}}
% \newcommand{\horizondisc}{k_{\regtext{f}}}
% \newcommand{\at}[1]{\!\left(#1\right)}
% \newcommand{\dt}{\Delta_t}

% \newcommand{\zonotope}{\set{Z}}
% \newcommand{\reachset}{\set{X}}
% \newcommand{\noisespace}{\set{W}}

% \newcommand{\statehistory}{X}
% \newcommand{\ctrlhistory}{U}

% % sizes of things
% \newcommand{\nstate}{{n_\state}}
% \newcommand{\nctrl}{{n_\ctrl}}
% \newcommand{\nnoise}{{n_\noise}}
% \newcommand{\nagents}{{n_{\regtext{a}}}}
% \newcommand{\nmodes}{{n_{\regtext{m}}}}
% \newcommand{\nego}{{n_{\ego}}}
% \newcommand{\ngen}{{n_{\regtext{g}}}}
% \newcommand{\ncon}{{n_{\regtext{c}}}}

% % zonotope stuff
% \newcommand{\zonofn}[1]{{\mathscr{Z}\!\left(#1\right)}}

% % MATS
% \newcommand{\MATS}{\phi}
% \newcommand{\param}{\theta}
